Harmonic Mean Density Fusion in Distributed Tracking: Performance and Comparison

A distributed sensor fusion architecture is preferred in a real target-tracking scenario as compared to a centralized scheme since it provides many practical advantages in terms of computation load, communication bandwidth, fault-tolerance, and scalability. In multi-sensor target-tracking literature, such systems are better known by the pseudonym - track fusion, since processed tracks are fused instead of raw measurements. A fundamental problem, however, in such systems is the presence of unknown correlations between the tracks, which renders a standard Kalman filter (naive fusion) useless. A widely accepted solution is covariance intersection (CI) which provides near-optimal estimates but at the cost of a conservative covariance. Thus, the estimates are pessimistic, which might result in a delayed error convergence. Also, fusion of Gaussian mixture densities is an active area of research where standard methods of track fusion cannot be used. In this article, harmonic mean density (HMD) based fusion is discussed, which seems to handle both of these issues. We present insights on HMD fusion and prove that the method is a result of minimizing average Pearson divergence. This article also provides an alternative and easy implementation based on an importance-sampling-like method without the requirement of a proposal density. Similarity of HMD with inverse covariance intersection is an interesting find, and has been discussed in detail. Results based on a real-world multi-target multi-sensor scenario show that the proposed approach converges quickly than existing track fusion algorithms while also being consistent, as evident from the normalized estimation-error squared (NEES) plots.

==> considered_corr_structure.tex <==
\subsection{Considered Correlation Structure in Track Fusion}
	
	A general form of independent and non-independent data-sets are shown in Fig. \ref{independentFig} and Fig. \ref{nonIndependentFig} 
	
	 \begin{figure}[h!]
	 	\centering
	 	\begin{tikzpicture}
	 		\draw(1,1) node[]{$\mathbf{x|z}^i$} ellipse(2cm and 0.5cm);
	 		\draw(5.5,1) node[]{$\mathbf{x|z}^j$} ellipse(2cm and 0.5cm);
	 	\end{tikzpicture}
	 	\caption{Independent Dataset}\label{independentFig}
	 \end{figure}
	 \begin{figure}[h!]
	 	\centering
	 	\begin{tikzpicture}
	 		\draw(1,1) node[]{$\mathbf{x|z}^{i/j}$} ellipse(2cm and 0.5cm);
	 		\draw(2.5,1) node[pin = above:{$\mathbf{x|z}^i\cap \mathbf{z}^j$}]{};
	 		\draw(4,1) node[]{$\mathbf{x|z}^{j/i}$} ellipse(2cm and 0.5cm);
	 	\end{tikzpicture}
	 	\caption{Non-independent Dataset \cite{julier2008fusion}}\label{nonIndependentFig}
	 \end{figure}
	 
	 Where the notation $\mathbf{z}^{i/j}$ denotes measurement data contained in node $i$ which is exclusive to node $j$. Using the concept of conditional independence depicted in Fig. \ref{nonIndependentFig} and the Bayes' theorem, the conditional density based on common information can be written as,
	 \begin{align}
	 	&P(\mathbf{x}|\mathbf{z}^i) = P(\mathbf{x|z}^{i/j})P(\mathbf{x}|\mathbf{z}^i\cap \mathbf{z}^j)\notag \\
	 	\Rightarrow &P(\mathbf{x}|\mathbf{z}^i\cap \mathbf{z}^j) = \frac{P(\mathbf{x}|\mathbf{z}^i)}{P(\mathbf{x|z}^{i/j})} \label{eq_gen_corr_struct}
	 	%\frac{P(\mathbf{z}^i|\mathbf{x})}{P(\mathbf{z}^i\cap \mathbf{z}^j)}\propto \frac{P(\mathbf{x}|\mathbf{z}^i)}{P(\mathbf{x}|\mathbf{z}^{i/j})},
	 \end{align}  
	Incorporating the information from another sensor and using the fact that $P(\mathbf{x}|\mathbf{z}^j\cap \mathbf{z}^i) = P(\mathbf{x}|\mathbf{z}^i\cap \mathbf{z}^j)$, it can be concluded that,
	\begin{align}
		P(\mathbf{x}|\mathbf{z}^i\cap \mathbf{z}^j) = \frac{1}{2} \frac{P(\mathbf{x}|\mathbf{z}^i)}{P(\mathbf{x}|\mathbf{z}^{i/j})} + \frac{1}{2} \frac{P(\mathbf{x}|\mathbf{z}^j)}{P(\mathbf{x}|\mathbf{z}^{j/i})}
	\end{align}
	which is clearly a mixture density. If we compare the Optimal Bayes distributed fusion equation in \eqref{exactBayesian} with that of HMD in eqn. \eqref{eq_HMD_gen}, it can be seen that the common information component in HMD matches the common information component for the correlation structure mentioned above. This is why, HMD is closest to Bayes optimal fusion result in comparison to all generalized conservative techniques.
	
	The correlation structure mentioned here is directly in-line with that presented in \cite{noack2017decentralized,noack2017inverse, sijs2010state} with the assumption of Gaussianity of all components. If $P(\mathbf{x}|\mathbf{z}^i\cap \mathbf{z}^j) = P(\mathbf{x}|\mathbf{z}^j\cap \mathbf{z}^i)$ are assumed to be Gaussian distributed as  $\mathcal{N}\left(\mathbf{x};\gamma_m, \mathbf{\Gamma}_m,\right)$, and the independent component in a track $P(\mathbf{x|z}^{i/j})$ is Gaussian as $\mathcal{N}\left(\mathbf{x};\gamma^i_\text{ind}, \mathbf{\Gamma}^i_\text{ind} \right)$, then the local track density is (using eqn. \eqref{eq_gen_corr_struct} ),
	\begin{align}
		P(\mathbf{x}|\mathbf{z}^i) &= P(\mathbf{x|z}^{i/j})P(\mathbf{x}|\mathbf{z}^i\cap \mathbf{z}^j) \notag \\
									&\propto \mathcal{N}\left(\mathbf{x}; \mathbf{\hat{x}}^i,\mathbf{\Gamma^i}\right) 
	\end{align}
	where
	\begin{align}
		\left(\mathbf{\Gamma}^i \right)^{-1} &= \left(\mathbf{\Gamma}^{-1}_m +  \left(\mathbf{\Gamma}^i_\text{ind}\right)^{-1} \right) \\
		\mathbf{\hat{x}}^i &= \mathbf{\Gamma}^i \left( \left(\mathbf{\Gamma}^i_\text{ind}\right)^{-1}  \mathbf{\gamma}^i_\text{ind} + \mathbf{\Gamma}^{-1}_m\mathbf{\gamma}_m \right) \label{eq_corr_struct}
	\end{align}
	which are the local track density parameters for Gaussian case. Similarly for the node $j$,
	\begin{align}
		\left(\mathbf{\Gamma}^j \right)^{-1} &= \left(\mathbf{\Gamma}^{-1}_m +  \left(\mathbf{\Gamma}^j_\text{ind}\right)^{-1} \right) \\
		\mathbf{\hat{x}}^j &= \mathbf{\Gamma}^j \left( \left(\mathbf{\Gamma}^j_\text{ind}\right)^{-1}  \mathbf{\gamma}^j_\text{ind} + \mathbf{\Gamma}^{-1}_m\mathbf{\gamma}_m \right)
	\end{align}
	If the mutual information component $\mathbf{\Gamma}_m, \mathbf{\gamma}_m $ is known, then the optimal fusion is simply the ratio of the product of local densities and the mutual information, as in eqn. \eqref{exactBayesian}. The result is,
	\begin{subequations}\label{eq_fusion_corr_struct}
	\begin{align}
		\mathbf{\Gamma}^f &= \left( \left( \mathbf{\Gamma}^i\right)^{-1} + \left( \mathbf{\Gamma}^j\right)^{-1} - \mathbf{\Gamma}^{-1}_m\right) \\
		\mathbf{\hat{x}}^f &= \left( \left( \mathbf{\Gamma}^i\right)^{-1}\mathbf{\hat{x}}^i + \left( \mathbf{\Gamma}^j\right)^{-1}\mathbf{\hat{x}}^j - \mathbf{\Gamma}^{-1}_m\mathbf{\gamma}_m \right)
 	\end{align}
 	\end{subequations}
	where $\mathbf{\Gamma}^f, \mathbf{\hat{x}}^f$ are the parameter of fused (Gaussian) density. 

	The resulting cross-correlation matrix according to the proposed correlation structure is,
	\begin{align}
		\mathbb{E}\left[\tilde{\mathbf{x}}^i\left(\tilde{\mathbf{x}}^j\right)^T \right] =  \mathbf{\Gamma}^i\mathbf{\Gamma}^{-1}_m\mathbf{\Gamma}^j\label{eq_crossCorr_struct}
	\end{align}	
	See appendix for proof. The fusion problem requires to approximate the consistent pair $\left(\mathbf{\gamma}_m,\Gamma_m\right)$ such that some criteria is satisfied.
